CWF: Consolidating Weak Features in High-quality Mesh Simplification

In mesh simplification, common requirements like accuracy, triangle quality, and feature alignment are often considered as a trade-off. Existing algorithms concentrate on just one or a few specific aspects of these requirements. For example, the well-known Quadric Error Metrics (QEM) approach prioritizes accuracy and can preserve strong feature lines/points as well but falls short in ensuring high triangle quality and may degrade weak features that are not as distinctive as strong ones. In this paper, we propose a smooth functional that simultaneously considers all of these requirements. The functional comprises a normal anisotropy term and a Centroidal Voronoi Tessellation (CVT) energy term, with the variables being a set of movable points lying on the surface. The former inherits the spirit of QEM but operates in a continuous setting, while the latter encourages even point distribution, allowing various surface metrics. We further introduce a decaying weight to automatically balance the two terms. We selected 100 CAD models from the ABC dataset, along with 21 organic models, to compare the existing mesh simplification algorithms with ours. Experimental results reveal an important observation: the introduction of a decaying weight effectively reduces the conflict between the two terms and enables the alignment of weak features. This distinctive feature sets our approach apart from most existing mesh simplification methods and demonstrates significant potential in shape understanding.

==> 8_add_figures.tex <==

\begin{figure*}[!t]
    \centering
    \begin{overpic}[width=0.98\linewidth]{figures/Comp_CAD.png}
\put( 4,-1.5){\textbf{CVT}}
\put(16,-1.5){\textbf{LpCVT}}
\put(30,-1.5){\textbf{QEM}}
\put(43,-1.5){\textbf{SMS}}
\put(55,-1.5){\textbf{IEM}}
\put(67,-1.5){\textbf{LPM}}
\put(79,-1.5){\textbf{Ours}}
\put(92,-1.5){\textbf{GT}}
    \end{overpic}
    \caption{
    Comparison with state of the arts on two CAD inputs. Our method surpasses other methods in both the accuracy and manifoldness of the reconstruction. Both point numbers are 500.
    }
    % \vspace{-2pt}
    \label{fig:comp_CAD}
\end{figure*}


\begin{figure*}[!t]
    \centering
    % \vspace{-2mm}
    \begin{overpic}[width=0.98\linewidth]{figures/Comp_bunny.png}
\put( 4.5,-1.5){\textbf{CVT}}
\put(18.5,-1.5){\textbf{LpCVT}}
\put(34,-1.5){\textbf{QEM}}
\put(49,-1.5){\textbf{SMS}}
\put(63,-1.5){\textbf{IEM}}
\put(78,-1.5){\textbf{LPM}}
\put(91,-1.5){\textbf{Ours}}

    \end{overpic}
    \caption{
    Comparison with state of the arts on the bunny model with 1000 sample points, our method can better consolidating the weak features.
    }
    % \vspace{-5pt}
    \label{fig:comp_organic}
\end{figure*}



\begin{figure*}[!t]
    \centering
    % \vspace{-2mm}
    \begin{overpic}[width=0.98\linewidth]{figures/weakFeature.png}
\put( 1,-1.5){\textbf{Base Surface}}
\put(16,-1.5){\textbf{CVT}}
\put(30,-1.5){\textbf{LpCVT}}
\put(43,-1.5){\textbf{QEM}}
\put(55,-1.5){\textbf{SMS}}
\put(67,-1.5){\textbf{IEM}}
\put(79,-1.5){\textbf{LPM}}
\put(92,-1.5){\textbf{Ours}}

    \end{overpic}
    \caption{
    Comparison with state of the arts on two smoothed inputs. Both sample point numbers are 500. Our method can better consolidating the weak features while the QEM-based methods will resulting in a chamfer along the feature line.
    }
    % \vspace{-5pt}
    \label{fig:comp_weak}
\end{figure*}

\clearpage



\begin{figure}[!t]
% \vspace{-5px}
\centering
\begin{overpic}
[width=0.99\linewidth]{figures/CompZT.png}
\put(7, -3) {VSR~\cite{zhao2023variational}}
\put(75, -3){Ours}

\end{overpic}
\caption{
Comparison with VSR~\cite{zhao2023variational}. Due to VSR is a QEM-based method that involves a mixed-integer programming step and practical success in finding a valid solution is not guaranteed. Numerous open mesh edges exist in this example due to the failure to satisfy manifold-edge constraints.
}
\label{fig:VSR}
% \vspace{-5pt}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{overpic}[width=0.95\linewidth]{figures/anisotropic_L}

    \put(10, 74.5){\textbf{(a) CVT}}
    \put(50, 74.5){\textbf{(b) Dual of (a)}}
    \put(10, 49){\textbf{(c) ACVT}}
    \put(50, 49){\textbf{(d) Dual of (c)}}
    \put(10, 23.5){\textbf{(e) CVT}}
    \put(50, 23.5){\textbf{(f) Dual of (e)}}
    \put(5, -2){\textbf{(g) Density-CVT}}
    \put(50, -2){\textbf{(h) Dual of (g)}}
    \end{overpic}
    \vspace{5pt}
    \caption{Examples of non-Euclidean distance, (a-d) is the anisotropic metrics and RVDs, (e-h) is the density-based metrics and RVDs.}
    \label{fig:anisotropic}
\end{figure}


% \begin{figure}[H]
% \centering
% \begin{overpic}
% [width=\linewidth]{figures/ablation.png}
% \put(7, 63) {$\mathbf{\lambda_{CVT}=0.1}$}
% \put(44,63) {$\mathbf{\lambda_{na}=0.1}$}
% \put(75, 63){$\mathbf{\tau=0.9}$}
% \put( 3, 33) {$\mathbf{\lambda_{CVT}=1.0}$\textbf{(Df.)}}
% \put( 40,33) {$\mathbf{\lambda_{na}=1.0}$\textbf{(Df.)}}
% \put(75, 33){$\mathbf{\tau=0.95}$\textbf{(Df.)}}
% \put( 7, 4) {$\mathbf{\lambda_{CVT}=10.0}$}
% \put(44, 4){$\mathbf{\lambda_{na}=10.0}$}
% \put(75, 4){$\mathbf{\tau=1.0}$}
% \end{overpic}
% \caption{
% Ablation study of the weighting coefficients $\tau$, $\lambda_{na}$ and $\lambda_{CVT}$, where bad edges are colored in red.
% We select
% $\tau=0.95$, $\lambda_{QEM}=1.0$, $\lambda_{CVT}=1.0$ as the favorite combination, which is used in all of our experiments.}
% \label{fig:ablation}
% \end{figure}




\begin{figure}[H]
\centering
\vspace{8pt}
\begin{overpic}
[width=0.99\linewidth]{figures/noise.png}
\put( 5, 63) {\textbf{{no-noise}}}
\put(38, 63) {\textbf{{$0.25\%$ noise}}}
\put(75, 63) {\textbf{{$0.50\%$ noise}}}
\put(-4, 3) {\rotatebox{90}{\textbf{Our Results}}}
\put(-4, 35){\rotatebox{90}{\textbf{Base Surface}}}
\end{overpic}
\caption{
Ablation study of our noise-resistant ability. We add $0.25\%$ and $0.50\%$ Gaussian noise to the surface vertices of the model. More noises may results in bad surface connectives such as self-intersections. Our method shows strong resistance to noise to some extent. }
\label{fig:noise}
\vspace{-5pt}
\end{figure}



\begin{figure}[H]
% \vspace{-5px}
\centering
\begin{overpic}
[width=0.99\linewidth]{figures/LowMesh.png}
\put(5, -3) {\textbf{Base Surface}}
\put(46, -3){\textbf{RVD}}
\put(79, -3){\textbf{Result}}

\end{overpic}
\caption{
Ablation study on low triangle quality of the based surface. The input mesh contains thin and sharp triangles which is normally undesired, our method shows resistance to these low-quality meshes as input, and outputs high-quality simplification result.
}
\label{fig:lowTri}
\vspace{-5pt}
\end{figure}


\begin{figure}[H]
% \vspace{-5px}
\centering
\begin{overpic}
[width=0.99\linewidth]{figures/openNumber.png}
\put(4, 25) {\textbf{Open Surface}}
\put(44, 25){\textbf{Our RVD}}
\put(75, 25){\textbf{Our Result}}
\put(7, -3) {$\mathbf{\#V=200}$}
\put(44, -3){$\mathbf{\#V=500}$}
\put(75, -3){$\mathbf{\#V=1000}$}
\end{overpic}
\caption{
Ablation study of input mesh with open surface (top) and three different sampling numbers of $\#V$ as target.
}
\label{fig:open_sampling}
\vspace{-5pt}
\end{figure}



